Second-Order Optimization via Quiescence

Second-order optimization methods exhibit fast convergence to critical points, however, in nonconvex optimization, these methods often require restrictive step-sizes to ensure a monotonically decreasing objective function. In the presence of highly nonlinear objective functions with large Lipschitz constants, increasingly small step-sizes become a bottleneck to fast convergence. We propose a second-order optimization method that utilizes a dynamic system model to represent the trajectory of optimization variables as an ODE. We then follow the quasi-steady state trajectory by forcing variables with the fastest rise time into a state known as quiescence. This optimization via quiescence allows us to adaptively select large step-sizes that sequentially follow each optimization variable to a quasi-steady state until all state variables reach the actual steady state, coinciding with the optimum. The result is a second-order method that utilizes large step-sizes and does not require a monotonically decreasing objective function to reach a critical point. Experimentally, we demonstrate the fast convergence of this approach for optimizing nonconvex problems in power systems and compare them to existing state-of-the-art second-order methods, including damped Newton-Raphson, BFGS, and SR1.

==> biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/Aayushya Agarwal _561.jpg}}]{Aayushya Agarwal} is a PhD candidate in the Department of Electrical and Computer Engineering at Carnegie Mellon University, where he is advised by Professor Lawrence Pileggi. Previously, he received his B.Sc degree from University of Waterloo in electrical and computer engineering. His research interests include optimization, power systems, machine learning and digital twins. 

\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/larry_photo.png}}]{Lawrence Pileggi} is the Coraluppi Head and the Tanoto Professor of Electrical and Computer Engineering at Carnegie Mellon. His work spans integrated circuit design, design automation, and simulation and optimization of energy systems. He co-founded Fabbrix Inc., Extreme DA, and Pearl Street Technologies. He has received several awards, including the Semiconductor Research Corporation Technical Excellence Awards in 1991 and 1999, the 2010 IEEE Circuits and Systems Society Mac Van Valkenburg Award, the 2015 Semiconductor Industry Association University Researcher Award, and the 2023 Phil Kaufman Award. He holds 41 U.S. patents and is a member of the National Academy of Inventors. He has published over 400 conference and journal papers. 
\end{IEEEbiography}



\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Figures/ron_picture.png}}]{Ron Rohrer} is Professor Emeritus of Electrical and Computer Engineering at Carnegie Mellon University.

Ron received the S.B. (1960) degree from Massachusetts Institute of Technology (MIT) and the M.S. (1961) and Ph.D. (1963) degrees from the University of California (UC) Berkeley
Ron was the 1981 founding editor of the IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems, and in 1988 served as president of the IEEE Circuits and Systems Society. He was elected Fellow of the IEEE in 1980 “for theoretical contributions and practical software for computer-aided circuit design.” In 1989 he was inducted into the National Academy of Engineering for contributions to circuit simulation that have enabled deep submicron IC design. He has authored five textbooks and over one hundred technical papers.  His many awards include a 1972-73 Alexander /Von Humboldt Senior Fellowship in its founding year, the 1978 ASEE Terman Award, the 1990 IEEE CAS Van Valkenburg Award, the 1990 SRC Inventor Recognition Award, the 1991 SRC Technical Excellence Award, the IEEE 1993 Education Medal “for innovation in bringing electrical engineering practice into the classroom and merging academic research with industrial need;” the 1996 NEC Computer and Communication Prize, a worldwide honor for pioneering contributions in electronics;  the 2002 Phil Kaufman award, presented by the EDA Consortium, the 2009 IEEE CAS Belevitch Award and the 2012 IEEE Kirchhoff Award.  

\end{IEEEbiography}

